Remote Sensing Vision-Language Foundation Models without Annotations via Ground Remote Alignment

We introduce a method to train vision-language models for remote-sensing images without using any textual annotations. Our key insight is to use co-located internet imagery taken on the ground as an intermediary for connecting remote-sensing images and language. Specifically, we train an image encoder for remote sensing images to align with the image encoder of CLIP using a large amount of paired internet and satellite images. Our unsupervised approach enables the training of a first-of-its-kind large-scale vision language model (VLM) for remote sensing images at two different resolutions. We show that these VLMs enable zero-shot, open-vocabulary image classification, retrieval, segmentation and visual question answering for satellite images. On each of these tasks, our VLM trained without textual annotations outperforms existing VLMs trained with supervision, with gains of up to 20% for classification and 80% for segmentation.

==> Tables/naip_clf_ret.tex <==
 \begin{table}
\small
\centering
      \caption{Zero-shot classification on the SAT-4 and SAT-6 benchmarks(left) and on our own dataset annotated with OSM (right). \cliprs outperforms the existing models on this modality as well. \\} \label{tab:naipcls}
      
      \begin{tabular}{l l r r | r } 
        \specialrule{.12em}{.1em}{.1em} 
        Model & Backbone & \multicolumn{1}{c}{SAT-4} & \multicolumn{1}{c}{SAT-6} & \multicolumn{1}{c}{NAIP-OSM} \\
        &  & Acc. & Acc &  mAP \\
        \specialrule{.12em}{.1em}{.1em} 

        CLIP & ViT-B/32& \sota{50.74} & \sota{30.39} & 26.94 \\
        CLIP & ViT-B/16& 46.60 & 25.82 & 31.89  \\
        CLIP-RSICD & ViT-B/32& 47.72 & 40.57 & \sota{32.51} \\
        RemoteCLIP & ViT-B/32& 33.55 & 20.76 & 23.29  \\
        \cmidrule{1-5}
        \textbf{\cliprs} & ViT-B/32 & \best{66.64} & \best{72.42} & 41.36 \\
        \textbf{\cliprs} & ViT-B/16& 53.42 & 66.57 & \best{42.47} \\
        \specialrule{.12em}{.1em}{.1em} 
      \end{tabular} 
\end{table}

\begin{table}
\small
\centering
      \caption{Text-based retrieval on our NAIP benchmark created using OSM data. \cliprs outperforms the existing models at this resolution as well. \\} \label{tab:naipret}
      
      \begin{tabular}{l l r r} 
        \specialrule{.12em}{.1em}{.1em} 
        Model & Backbone & \multicolumn{2}{c}{NAIP-OSM} \\
        &   & mAP@100  & mAP@20\\
        \specialrule{.12em}{.1em}{.1em} 

        CLIP & ViT-B/32&  56.71 & 57.51\\
        CLIP & ViT-B/16&  60.88 & 61.59 \\
        CLIP-RSICD & ViT-B/32&  \sota{64.58} & \sota{63.71}\\
        RemoteCLIP & ViT-B/32&  42.03 & 40.84 \\
        \cmidrule{1-4}
        \textbf{\cliprs} & ViT-B/32 &  74.31 & 74.77\\
        \textbf{\cliprs} & ViT-B/16&  \best{75.35} & \best{76.55}\\
        \specialrule{.12em}{.1em}{.1em} 
      \end{tabular} 
\end{table}




==> Tables/segment.tex <==
\begin{table}
    \parbox{.5\linewidth}{
    \centering  
    \begin{tabular}{l r r} 
        \specialrule{.12em}{.1em}{.1em} 
        Model & \multicolumn{1}{c}{NAIP} & \multicolumn{1}{c}{Sentinel}\\
        \specialrule{.12em}{.1em}{.1em} 
        CLIPSeg & \second{26.99} & \second{20.02}\\
        \cmidrule{1-4}
        \textbf{\cliprs} & \best{49.38} & 31.95\\
        \textbf{\cliprs+SAM} & - & \best{32.43}\\
        \specialrule{.12em}{.1em}{.1em} 
      \end{tabular} 
    }

  \caption{Per-class accuracy of our pixel-level models on the Satlas land-cover segmentation task.} \label{tab:segmentation}
\end{table}

==> Tables/segmentsen.tex <==
\begin{table}
    \parbox{.5\linewidth}{
    \centering  
    \begin{tabular}{l r} 
        \specialrule{.12em}{.1em}{.1em} 
        Model & \multicolumn{2}{c}{Satlas-seg}\\
         & Per Class Acc.\\
        \specialrule{.12em}{.1em}{.1em} 
        CLIPSeg & 20.02\\
        \cmidrule{1-3}
        \cliprs & 31.95\\
        \textbf{\cliprs+SAM} & 32.43\\
        \specialrule{.12em}{.1em}{.1em} 
      \end{tabular} 
    }

  \caption{(Left) } \label{tab:segmentation}
\end{table}

==> Tables/sentinel_clf_ret.tex <==
\begin{table}
\small
\centering
      \caption{Classification results on Sentinel-2 datasets. We measure zero-shot performance for the VLMs and one-shot performance for the representation learning techniques. Our model is significantly better on both datasets. 
      \\
      } \label{tab:clssent}
      \begin{tabular}{l c l l r r} 
        \specialrule{.12em}{.1em}{.1em} 
        Model & Labeled & Shot & Backbone & EuroSAT & BigEarthNet \\
        & Satellite & &  & Acc. & mAP \\
        &Data & &  & & \\
        \specialrule{.12em}{.1em}{.1em} 
        CLIP & \xmark & \multirow{4}{*}{0-shot} & ViT-B/32 & 47.61 & 21.31 \\
        CLIP & \xmark & & ViT-B/16& \sota{53.59}  & 23.13 \\
        CLIP-RSICD & \cmark & &  ViT-B/32 & 45.93  & \sota{27.68} \\
        RemoteCLIP & \cmark & & ViT-B/32& 38.59  & 22.76 \\
        \cmidrule{1-6}
        SeCo & \xmark & \multirow{3}{*}{1-shot}& ResNet-50& 45.63 &  23.86 \\
        CACo & \xmark &  & ResNet-50& 48.50  & 26.92 \\
        Satlas & \cmark & & Swin& 42.04  & 18.47 \\
        \cmidrule{1-6}
        \textbf{\cliprs}&  \xmark & \multirow{2}{*}{0-shot} & ViT-B/32 & 47.80  & 29.31 \\
        \textbf{\cliprs}&  \xmark & & ViT-B/16& \best{63.76}  & \best{32.46} \\
        \specialrule{.12em}{.1em}{.1em} 
      \end{tabular} 
\end{table}


\begin{table}
\small
\centering
\caption{Image retrieval performance on Sentinel-2 datasets. We use text-based retrieval for VLMs and image-based retrieval for the representation learning approaches. Our model outperforms all baselines.
      \\
      } \label{tab:retsent}
\begin{tabular}{l c l l r r |  r r} 
        \specialrule{.12em}{.1em}{.1em} 
        Model & Labeled & Query & Backbone & \multicolumn{2}{c}{EuroSAT} & \multicolumn{2}{c}{BigEarthNet} \\
        & Satellite & &  . & \multicolumn{2}{c}{mAP@}  & \multicolumn{2}{c}{mAP@}\\
        &Data & & & 100 & 20 & 100  & 20\\
        \specialrule{.12em}{.1em}{.1em} 
        CLIP & \xmark & \multirow{4}{*}{Text} & ViT-B/32  & 46.86 & 49.61  & 30.45 & 32.20\\
        CLIP & \xmark & & ViT-B/16 & 63.99 & 72.57  & 32.54 & 33.10\\
        CLIP-RSICD & \cmark & &  ViT-B/32  & 49.88 & 53.50  & 38.76 & 36.11\\
        RemoteCLIP & \cmark & & ViT-B/32 & 51.21 & 53.27  & 34.39 & 38.42\\
        \cmidrule{1-8}
        SeCo & \xmark & \multirow{3}{*}{Image}& ResNet-50& 68.78 & 78.42  & 40.48 & 51.11\\
        CACo & \xmark &  & ResNet-50 & \sota{69.90} & \sota{79.15}  & \sota{47.40} & \best{57.02}\\
        Satlas & \cmark & & Swin & 63.64 & 72.61  & 29.17 & 30.46\\
        \cmidrule{1-8}
        \textbf{\cliprs}&  \xmark & \multirow{2}{*}{Text} & ViT-B/32  & 66.12 & 72.36  & 45.88 & 45.35\\
        \textbf{\cliprs}&  \xmark & & ViT-B/16 & \best{81.56} & \best{85.21} & \best{49.61} & \second{53.86}\\
        \specialrule{.12em}{.1em}{.1em} 
      \end{tabular}



\end{table}
